Converting an Integer to a Decimal String in Under Two Nanoseconds

Converting binary integers to variable-length decimal strings is a fundamental operation in computing. Conventional fast approaches rely on recursive division and small lookup tables. We propose a SIMD-based algorithm that leverages integer multiply-add instructions available on recent AMD and Intel processors. Our method eliminates lookup tables entirely and computes multiple quotients and remainders in parallel. Additionally, we introduce a dual-variant design with dynamic selection that adapts to input characteristics: a branch-heavy variant optimized for homogeneous digit-length distributions and a branch-light variant for heterogeneous datasets. Our single-core algorithm consistently outperforms all competing methods across the full range of integer sizes, running 1.4-2x faster than the closest competitor and 2-4x faster than the C++ standard library function std::to_chars across tested workloads.

==> results/table_algorithm_comparison_clang++.tex <==
\begin{table}
  \caption{Performance comparison of integer-to-string algorithms across datasets.
  Metrics: ns/n = nanoseconds, i/n = instructions, c/n = cycles per number.
  \textbf{Bold} indicates fastest; \% shows difference vs Champagne--Lemire (positive = slower).}%
  \label{tab:algorithm_comparison}
  \centering
  \small
  \begin{tabular}{llrrrrrr}
    \toprule
    Algorithm & Dataset & ns/n & \% & i/n & \% & c/n & \% \\
    \midrule
    \rowcolor{black!10}
    Champagne--Lemire & \textbf{Twitter JSON} & 0.93 & - & 31.5 & - & 5.32 & - \\
    \rowcolor{black!10}
     & \textbf{CIT Patents} & 0.95 & - & 34 & - & 5.15 & - \\
    \rowcolor{black!10}
     & \textbf{Natural 1-8 digit} & 1.08 & - & 27.2 & - & 6.03 & - \\
    \rowcolor{white}
    jeaiii & Twitter JSON & 1.24 & +33.3 & 35.8 & +13.5 & 7.04 & +32.3 \\
    \rowcolor{white}
     & CIT Patents & 1.33 & +40.0 & 46 & +35.3 & 7.29 & +41.6 \\
    \rowcolor{white}
     & Natural 1-8 digit & 1.32 & +22.2 & 46 & +69.0 & 7.33 & +21.6 \\
    \rowcolor{black!10}
    yy & Twitter JSON & 1.45 & +55.9 & 43.9 & +39.3 & 8.19 & +53.9 \\
    \rowcolor{black!10}
     & CIT Patents & 1.83 & +92.6 & 53 & +55.9 & 10.1 & +96.3 \\
    \rowcolor{black!10}
     & Natural 1-8 digit & 1.83 & +69.4 & 53 & +94.7 & 10.1 & +68.0 \\
    \rowcolor{white}
    AppNexus & Twitter JSON & 2.24 & +140.9 & 50.8 & +61.2 & 12.7 & +137.8 \\
    \rowcolor{white}
     & CIT Patents & 2.99 & +214.7 & 64 & +88.2 & 16.8 & +225.4 \\
    \rowcolor{white}
     & Natural 1-8 digit & 2.99 & +176.9 & 64 & +135.1 & 16.8 & +177.8 \\
    \rowcolor{black!10}
    Abseil FastInt & Twitter JSON & 2.31 & +148.4 & 60.7 & +92.5 & 13 & +144.7 \\
    \rowcolor{black!10}
     & CIT Patents & 3.16 & +232.6 & 85 & +150.0 & 17.6 & +242.7 \\
    \rowcolor{black!10}
     & Natural 1-8 digit & 3.4 & +214.8 & 86.9 & +219.4 & 19 & +214.8 \\
    \rowcolor{white}
    std::to\_chars & Twitter JSON & 2.02 & +117.2 & 65.3 & +107.1 & 11.4 & +114.1 \\
    \rowcolor{white}
     & CIT Patents & 2.87 & +202.1 & 99 & +191.2 & 16 & +210.1 \\
    \rowcolor{white}
     & Natural 1-8 digit & 3.05 & +182.4 & 102 & +274.3 & 16.9 & +179.4 \\
    \rowcolor{black!10}
    Mathisen SSE & Twitter JSON & 2.05 & +120.4 & 59.3 & +88.1 & 11.6 & +117.9 \\
    \rowcolor{black!10}
     & CIT Patents & 3.99 & +320.0 & 108 & +217.6 & 22.2 & +330.3 \\
    \rowcolor{black!10}
     & Natural 1-8 digit & 4.19 & +288.0 & 102 & +275.4 & 23.3 & +287.1 \\
    \rowcolor{white}
    Hopman & Twitter JSON & 3.43 & +268.8 & 90.8 & +187.9 & 19.3 & +262.4 \\
    \rowcolor{white}
     & CIT Patents & 3.86 & +306.3 & 119 & +250.0 & 21.4 & +315.7 \\
    \rowcolor{white}
     & Natural 1-8 digit & 3.95 & +265.7 & 116 & +326.5 & 21.9 & +262.7 \\
    \rowcolor{black!10}
    Naive & Twitter JSON & 3.22 & +246.2 & 86.3 & +173.8 & 18.1 & +240.8 \\
    \rowcolor{black!10}
     & CIT Patents & 4.89 & +414.7 & 117 & +244.1 & 27.4 & +432.4 \\
    \rowcolor{black!10}
     & Natural 1-8 digit & 4.74 & +338.9 & 120 & +340.4 & 26.6 & +341.0 \\
    \bottomrule
  \end{tabular}\restartrowcolors
\end{table}

==> results/table_algorithm_comparison_g++.tex <==
\begin{table}
  \caption{Performance comparison of integer-to-string algorithms across datasets.
  Metrics: ns/n = nanoseconds, i/n = instructions, c/n = cycles per number.
  \textbf{Bold} indicates fastest; \% shows difference vs Champagne--Lemire (positive = slower).}%
  \label{tab:algorithm_comparison}
  \centering
  \small
  \begin{tabular}{llrrrrrr}
    \toprule
    Algorithm & Dataset & ns/n & \% & i/n & \% & c/n & \% \\
    \midrule
    \rowcolor{black!10}
    Champagne--Lemire & \textbf{Twitter JSON} & 1.12 & - & 37.7 & - & 6.38 & - \\
    \rowcolor{black!10}
     & \textbf{CIT Patents} & 1.06 & - & 39 & - & 5.78 & - \\
    \rowcolor{black!10}
     & \textbf{Natural 1-8 digit} & 0.93 & - & 30.3 & - & 5.04 & - \\
    \rowcolor{white}
    jeaiii & Twitter JSON & 1.26 & +12.5 & 41.4 & +9.9 & 7.12 & +11.6 \\
    \rowcolor{white}
     & CIT Patents & 1.49 & +40.6 & 54 & +38.5 & 8.15 & +41.0 \\
    \rowcolor{white}
     & Natural 1-8 digit & 1.47 & +58.1 & 54 & +78.3 & 8.02 & +59.1 \\
    \rowcolor{black!10}
    yy & Twitter JSON & 1.45 & +29.5 & 43.9 & +16.4 & 8.21 & +28.7 \\
    \rowcolor{black!10}
     & CIT Patents & 1.82 & +71.7 & 55 & +41.0 & 10.1 & +74.6 \\
    \rowcolor{black!10}
     & Natural 1-8 digit & 1.82 & +95.7 & 55 & +81.6 & 10.1 & +99.8 \\
    \rowcolor{white}
    AppNexus & Twitter JSON & 1.87 & +67.0 & 44.8 & +18.8 & 10.6 & +66.0 \\
    \rowcolor{white}
     & CIT Patents & 2.51 & +136.8 & 56 & +43.6 & 14.1 & +143.1 \\
    \rowcolor{white}
     & Natural 1-8 digit & 2.5 & +168.8 & 56 & +84.9 & 14.1 & +178.8 \\
    \rowcolor{black!10}
    Abseil FastInt & Twitter JSON & 2.25 & +100.9 & 65.7 & +74.3 & 12.7 & +99.2 \\
    \rowcolor{black!10}
     & CIT Patents & 3.23 & +204.7 & 96 & +146.2 & 18.1 & +213.0 \\
    \rowcolor{black!10}
     & Natural 1-8 digit & 3.18 & +241.9 & 90.2 & +197.8 & 17.7 & +252.0 \\
    \rowcolor{white}
    std::to\_chars & Twitter JSON & 1.95 & +74.1 & 69.2 & +83.5 & 11 & +72.3 \\
    \rowcolor{white}
     & CIT Patents & 2.76 & +160.4 & 108 & +176.9 & 15 & +159.5 \\
    \rowcolor{white}
     & Natural 1-8 digit & 3.11 & +234.4 & 114 & +275.8 & 16.9 & +234.3 \\
    \rowcolor{black!10}
    Mathisen SSE & Twitter JSON & 2.5 & +123.2 & 61.9 & +64.3 & 14.1 & +121.3 \\
    \rowcolor{black!10}
     & CIT Patents & 4.3 & +305.7 & 100 & +156.4 & 24 & +315.4 \\
    \rowcolor{black!10}
     & Natural 1-8 digit & 4.83 & +419.4 & 103 & +239.9 & 27.1 & +437.5 \\
    \rowcolor{white}
    Hopman & Twitter JSON & 3.17 & +183.0 & 85.2 & +126.2 & 17.9 & +180.3 \\
    \rowcolor{white}
     & CIT Patents & 4.2 & +296.2 & 113 & +189.7 & 23.5 & +306.4 \\
    \rowcolor{white}
     & Natural 1-8 digit & 4.37 & +369.9 & 111 & +266.8 & 24.5 & +385.9 \\
    \rowcolor{black!10}
    Naive & Twitter JSON & 3.48 & +210.7 & 85.5 & +126.8 & 19.6 & +207.2 \\
    \rowcolor{black!10}
     & CIT Patents & 4.66 & +339.6 & 120 & +207.7 & 26 & +350.0 \\
    \rowcolor{black!10}
     & Natural 1-8 digit & 5.38 & +478.5 & 135 & +344.3 & 30 & +496.0 \\
    \bottomrule
  \end{tabular}\restartrowcolors
\end{table}

==> results/table_homogeneous_vs_heterogeneous_g++.tex <==
\begin{table}
  \caption{Performance comparison of homogeneous vs heterogeneous variants
  across different datasets. Times shown in nanoseconds per number (ns/n).
  The \textbf{bold} value indicates the faster variant for each dataset.
  The ``Selected'' column shows which variant was chosen by auto-detection.}%
  \label{tab:homogeneous_vs_heterogeneous}
  \centering
  \begin{tabular}{lrrr}
    \toprule
    Dataset & Homogeneous (ns/n) & Heterogeneous (ns/n) & Selected \\
    \midrule
    Uniform 4-digit (1M) & \textbf{0.75} & 1.03 & Homo \\
    Uniform 8-digit (1M) & \textbf{0.75} & 0.96 & Homo \\
    Uniform 16-digit (1M) & \textbf{1.12} & 1.43 & Homo \\
    Uniform 1-20 digits (1M) & 7.55 & \textbf{4.87} & Hetero \\
    Natural-8 (1M) & \textbf{0.93} & 0.96 & Homo \\
    Natural-16 (1M) & \textbf{1.32} & 1.49 & Homo \\
    CITM Catalog & 1.65 & \textbf{1.53} & Homo \\
    Twitter JSON & \textbf{0.99} & 1.12 & Hetero \\
    StackOverflow Timestamps & 1.59 & \textbf{1.44} & Homo \\
    US Patents & 1.06 & \textbf{0.98} & Homo \\
    \bottomrule
  \end{tabular}\restartrowcolors
\end{table}
